On Fully Dynamic Graph Sparsifiers

We initiate the study of dynamic algorithms for graph sparsification problems and obtain fully dynamic algorithms, allowing both edge insertions and edge deletions, that take polylogarithmic time after each update in the graph. Our three main results are as follows. First, we give a fully dynamic algorithm for maintaining a $ (1 \pm \epsilon) $-spectral sparsifier with amortized update time $poly(\log{n}, \epsilon^{-1})$. Second, we give a fully dynamic algorithm for maintaining a $ (1 \pm \epsilon) $-cut sparsifier with \emph{worst-case} update time $poly(\log{n}, \epsilon^{-1})$. Both sparsifiers have size $ n \cdot poly(\log{n}, \epsilon^{-1})$. Third, we apply our dynamic sparsifier algorithm to obtain a fully dynamic algorithm for maintaining a $(1 + \epsilon)$-approximation to the value of the maximum flow in an unweighted, undirected, bipartite graph with amortized update time $poly(\log{n}, \epsilon^{-1})$.

==> cut_sparsifier_worst_case.tex <==
\subsection{Dynamic Cut Sparsifier with Amortized Update Time}\label{sec:cut sparsifier amortized}

We now explain how to implement the cut sparsifier of \Cref{sec:cut sparsifier general} dynamically.
The main building block of our algorithm is the fully dynamic algorithm of Holm, de Lichtenberg, and Thorup~\cite{HolmLT01}.
We need the following additional property for bounding the number of changes to the spanning tree, which follows from the fact that the minimum spanning tree of Holm et al.~\cite{HolmLT01} is repaired after a deletion by finding a single replacement edge.

\begin{theorem}[\cite{HolmLT01}]
	There is a fully dynamic deterministic algorithm for maintaining a minimum spanning forest $ F $ of a weighted undirected graph $ G $ with amortized update time $ O (\log^4{n}) $.
	Every time an edge $ e $ is inserted into $ G $, the only potential change to $ F $ is the insertion of $ e $ and if so possibly the removal at most one other edge $ F $.
	Every time an edge $ e $ is deleted from $ G $, the only potential change to $ F $ is the removal of $ e $ and possibly the addition of at most one other edge to $ F $.
\end{theorem}

By negating the edge weights this algorithm can as well be used for maintaining a maximum spanning tree, which using the terminology introduced above is a $1$-MST of size $ O (n) $.
We now show how we use this algorithm for maintaining a $t$-bundle $1$-MST and consequently a $ (1 \pm \epsilon) $ cut sparsifier $ H $ according to the construction presented in \Cref{sec:cut sparsifier general}.

We maintain a $t$-bundle $1$-MST $ B = \bigcup_{1 \leq i \leq k} T_i $ by maintaining, for every $ 1 \leq i \leq k $, a maximum spanning tree of $ G \setminus \bigcup_{j=1}^{i-1} T_j $.
We now analyze how changes to $ G \setminus \bigcup_{j=1}^{i-1} T_j $ affect $ G \setminus \bigcup_{j=1}^i T_j $ (for every $ 1 \leq i \leq k $):
\begin{itemize}
	\item Whenever an edge $ e $ is inserted into $ G \setminus \bigcup_{j=1}^{i-1} T_j $, the maximum spanning tree algorithm either adds $ e $ to $ T_i $ (possibly replacing some edge $ f $) or not.
	\begin{itemize}
		\item If $ e $ is added to $ T_i $ and $ f $ is removed from $ T_i $, then $ f $ is added to $ G \setminus \bigcup_{j=1}^i T_j $.
		\item If $ e $ is not added to $ T_i $, then $ e $ is added to $ G \setminus \bigcup_{j=1}^i T_j $.
	\end{itemize}
	\item Whenever an edge $ e $ is deleted from $ G \setminus \bigcup_{j=1}^{i-1} T_j $, either $ e $ is contained in $ T_i $ or not.
	\begin{itemize}
		\item If $ e $ is contained in $ T_i $, then the maximum spanning tree algorithm will remove $ e $ from $ H $ and add some other edge $ f $ to $ T_i $.
		This edge $ f $ will be removed from $ G \setminus \bigcup_{j=1}^i T_j $.\footnote{The edge $ e $ will not be added to $ G \setminus \bigcup_{j=1}^i T_j $ because it is removed from both $ G \setminus \bigcup_{j=1}^{i-1} T_j $ and $ T_i $.}
		\item If $ e $ is not contained in $ T_i $, then $ e $ is removed from $ G \setminus \bigcup_{j=1}^i T_j $.
	\end{itemize}
\end{itemize}
Thus, every change to $ G \setminus \bigcup_{j=1}^{i-1} T_j $ results in one change to $ G \setminus \bigcup_{j=1}^i T_j $.
Consequently, a single update to~$ G $ results to at most one update in each instance of the dynamic MST algorithm.
For every update in $ G $ we therefore incur an amortized update time of $ O (t \log^4{n}) $.
We can summarize the guarantees for maintaining $t$-bundle $1$-MSTs as follows.

\begin{corollary}
There is a fully dynamic algorithm for maintaining a $t$-bundle $1$-max-spanner $ B $ (where $ t \geq 1 $ is an integer) of size $ O (t n) $ with amortized update time $ O (t \log^4{n}) $.
After every update of $ G $, the graph $ G \setminus B $ changes by at most one edge.
\end{corollary}

Finally, we explain how to maintain the cut sparsifier.
We use $ l = \lceil \log{\rho} \rceil $ instances of the dynamic $t$-bundle $1$-max-spanner algorithm above to maintain iteratively, for every $ 1 \leq i \leq k $, a $t$-bundle spanner $ B_i $ of a graph $ G_i $.
For every $ 1 \leq i \leq k $, the graph $ G_i $ is maintained as follows:
\begin{itemize}
	\item Whenever an edge $ e $ is inserted into $ G_i $ and it is not added to $ B_i $, then it is added to $ G_{i+1} $ with probability $ 1/2 $.
	\item Whenever an edge $ e $ is removed from $ G_i $ and it has not been deleted from $ G $, then it is added to $ G_{i+1} $ with probability $ 1/2 $.
	\item Whenever an edge $ e $ is deleted from $ G $, it is removed from $ G_i $ if contained.
\end{itemize}
Note that with every update in $ G $ there is at most one update to every $ G_i $.
Thus, the amortized update time for maintaining each is $ O (t \log^4{n}) $ per deletion in $ G $.

Finally, observe that the cut sparsifier $ H $ consists of a collection of bundles, which in turn consists of a collection of trees. Thus, the cut sparsifier has low arboricity and we can maintain the collection of trees it consists of explicitly.\sebastian{TODO: The statment is not true yet. If we want the sparsifier to consist of only trees we cannot really use the density parameter $ \rho $}
Our algorithm therefore provides the following guarantees.

\begin{theorem}
There is a fully dynamic algorithm for maintaining a $ (1 \pm \epsilon) $-cut sparsifier $ H $ of size $ \tilde O (n) $ of a weighted undirected graph $ G $ that has an amortized update time of $ \tilde O (1) $.
The cut sparsifier $ H $ has arboricity $ \tilde O (1) $ and the algorithm explicitly maintains $ H $ as a collection of $ \tilde O (1) $ forests.\sebastian{Anything else we need for the vertex cover algorithm? Storing the degree in each forest so that we know the leaves?}
The algorithm is correct with high probability against an oblivious adversary.
\end{theorem}

\begin{comment}
Fung et al.\ showed how that a cut sparsifier can be obtained by sampling edges according to their local connectivities.
For their algorithm to work it is sufficient to have suitable estimate for the connectivities.
In particular they use the so-called \emph{Nagamochi-Ibaraki indices} as estimates for the connectivites.
Nagamochi and Ibaraki devised an algorithm for partitioning the graph into a sequence of maximal spanning forests.
A set of edge-disjoint spanning forests $ T_1, T_2, \dots, T_k $ is called a \emph{Nagamochi-Ibaraki (NI) forest} packing if, for every $ 1 \leq i \leq k $, $ T_i $ is a spanning forest of $ G \setminus \bigcup_{j=1}^{i-1} T_j $.
The \emph{Nagamochi-Ibaraki index} of an edge $ e $ is the index of the last NI forest in which $ e $ appears.

A simple-minded approach for dynamically maintaining a cut sparsifier would be to maintain the Nagamochi-Ibaraki indices using the dynamic connectivity algorithm of Holm et al.~\cite{HolmLT01}

We are not aware of any algorithm specifically designed for this problem.
A straigthforward idea would be to use the dynamic connectivity algorithm of Holm et al.~\cite{HolmLT01} for this task.
However, if we do this naively, we need up to $ n $ instances of this algorithm, one for each spanning tree.
\end{comment}


\subsection{Dynamic Cut Sparsifier with Worst-Case Update Time}

We now extend the result to worst-case udpate time.
This can be done at the cost of slightly worse guarantees, with an additional dependence on $ \log{W} $ in the size, than in the amortized case by using the worst-case connectivity data structure of Kapron, King, and Mountjoy~\cite{KapronKM13}.
Remember that $ W $ is the ratio between the largest and the smallest edge weight in $ G $.
In the following we assume without loss of generality that the edge weights of $ G $ are integers in the range from $ 1 $ to $ W $.
This can be achieved by rescaling the edge weights.

It is not known whether a minimum/maximum spanning forest can be maintained fully dynamically with polylogarithmic worst-case update time.
However we can get an approximate version of the MST that is good enough for our purposes by using the following spanning tree algorithm.

\begin{theorem}[\cite{KapronKM13,GibbKKT15}]\label{thm:worst case connectivity}
	There is a fully dynamic deterministic algorithm for maintaining a spanning forest $ F $ of an undirected graph $ G $ with worst-case update time $ O (log^4{n}) $.
	Every time an edge $ e $ is inserted into $ G $, the only potential change to $ F $ is the insertion of $ e $ and if so possibly the removal at most one other edge $ F $.
	Every time an edge $ e $ is deleted from $ G $, the only potential change to $ F $ is the removal of $ e $ and possibly the addition of at most one other edge to $ F $.
	The algorithm is correct with high probability against an oblivious adversary.
\end{theorem}

We now explain how we use this data structure in a straightforward way to maintain a $2$-MST with worst-case update time under edge deletions in $ G $.\sebastian{The SODA'13 paper claims that the worst-case connectivity data structure can be used to maintain (the weight of) an approximate MST, using a reduction of Henzinger/King JACM'99. However, I don't believe that this will work. It seems that the reduction can only safely be used for deterministic algorithms. For us this means that if want worst-case update time we have logarithmic dependence on the edge weights in both the size of the sparsifier and the update time.}
For every $ 0 \leq i \leq \lfloor \log W \rfloor $, let $ E_i $ be the set of edges of weight between $ 2^i $ and $ 2^{i+1} $, i.e., $ E_i = \{ e \in E \mid 2^i \leq \ww_G (e) < 2^{i+1} \} $, and run a separate instance of the connectivity algorithm of \Cref{thm:worst case connectivity} for the edges in $ E_i $.
For every $ 0 \leq i \leq \lfloor \log W \rfloor $, let $ T_i $ be the spanning forest of the edges in $ E_i $ maintained by the $i$-th instance of the connectivity data structure.
We claim that the union of all these trees is a $2$-MST of $ G $.

\begin{lemma}
$ H = \bigcup_{i=0}^{\lfloor \log W \rfloor} T_i $ is a $2$-MST of $ G $.
\end{lemma}

\begin{proof}
Consider some edge $ e = (u, v) $ of $ G $ and let $ i $ be the (unique) index such that $ 2^i \leq \ww_G (e) < 2^{i+1} $.
Since $ T_i $ is spanning tree of $ G $, there is a path $ \pi $ from $ u $ to $ v $ in $ T_i $ (and thus also in $ H $).
Every edge $ f $ of $ \pi $ is in the same weight class as $ e $, i.e., $ 2^i \leq \ww_G (f) < 2^{i+1} $.
Thus, $ \ww_G (e) < 2^{i+1} \leq 2 \ww_G (f) $ as desired.
\end{proof}

At the initialization we partition the edges into the weight classes as above and then for every $ 0 \leq i \leq \lfloor \log W \rfloor $ we insert every edge of $ E_i $ into the $i$-th instance of the connectivity algorithm
Every time an edge $ e $ is deleted, we determine the weight class $ i $ of $ e $ and perform the deletion in the $i$-th instance of the connectivity algorithm.
In this way we get a worst-case running time of $ O (\log^4{n}) $ per edge during the deletions and the preprocessing.

\begin{corollary}
There is a fully dynamic algorithm for maintaining a $2$-MST $ H $ of size $ O (n \log{W}) $ of a graph $ G $ with positive edge weights that has a preprocessing time of $ O (m \log^4{n}) $ and a worst-case update time of $ O (\log^4{n}) $, where $ W $ is the ratio between the largest and the smallest edge weight.
Every time the algorithm inserts an edge into $ H $ it stays in $ H $ until it is deleted from $ G $ as well.
\end{corollary}

Now we simply follow the same steps as in \Cref{sec:cut sparsifier amortized} to get the desired sparsifier.
The high-probability bounds of the algorithm hold for a polynomially bounded sequence of updates.
We explain how to get rid of this technical restriction in \Cref{lem:arbitrarily long sequences}.

\begin{theorem}
There is a fully dynamic algorithm for maintaining a $ (1 \pm \epsilon) $-cut sparsifier $ H $ of size $ \tilde O (n \log{W}) $ of a weighted undirected graph $ G $ that has an worst-case update time of $ \tilde O (1) $.
The cut sparsifier $ H $ has arboricity $ \tilde O (1) $ and the algorithm explicitly maintains $ H $ as a collection of $ \tilde O (1) $ forests.
The algorithm is correct with high probability against an oblivious adversary.
\end{theorem}


\subsection{Handling Arbitrarily Long Sequences of Updates}\label{lem:arbitrarily long sequences}

The high-probability guarantees of the algorithm above only holds for a polynomially bounded number of updates.
We now show how to extend it to an arbitrarily long sequence of updates providing the same asymptotic update time and size of the sparsifier.
We do this by concurrenlty running two instances of the dynamic algorithm that periodically take turns in being restarted, which is a fairly standard approach for such situations.
The only new aspect necessary for our purposes is that both instances explicitly maintain a sparsifier and when taking turns we cannot simply replace all the edges of one sparsifier with the edges of the other sparsifier as processing all these edges would violate the worst-case update time guarantee.
For this reason we exploit the decomposability of graph sparsifiers and maintain a `blend' of the two sparsifiers computed by the concurrent instances of the dynamic algorithm.
This step is not necessary for other dynamic problems such as connectivitz where we only have to make sure that the query is delegated to the currently active instance. % TODO cite??

\begin{lemma}[Decomposability]\label{lem:decomposability cut sparsifier}
Let $ G = (V, E) $ be an undirected weighted graph, let $ E_1, \dots, E_k $ be a partition of the set of edges $E$, and let, for every $ 1 \leq i \leq k $, $ H_i $ be a $ (1 \pm \epsilon) $-cut sparsifier of $ G_i = (V, E_i) $.
Then $ H = \bigcup_{i=1}^k H_i $ is a $ (1 \pm \epsilon) $-cut sparsifier of $ G $.
\end{lemma}

\begin{proof}
Let $ U $ be a cut in $ G $.
First observe that
\begin{equation*}
\ww_G (\partial_G (U)) = \ww_G (\bigcup_{i=1}^k \partial_{G_i} (U)) = \sum_{i=1}^k \ww_G (\partial_{G_i} (U)) = \sum_{i=1}^k \ww_{G_i} (\partial_{G_i} (U))
\end{equation*}
and similarly $ \ww_H (\partial_H (U)) = \sum_{i=1}^k \ww_{H_i} (\partial_{H_i} (U)) $.
Now since
\begin{equation*}
	(1 - \epsilon) \ww_{H_i} (\partial_{H_i} (U)) \leq \ww_{G_i} (\partial_{G_i} (U)) \leq (1 + \epsilon) \ww_{H_i} (\partial_{H_i} (U))
\end{equation*} 
for every $ 1 \leq i \leq k $, we have
\begin{multline*}
	(1 - \epsilon) \ww_H (\partial_H (U)) = (1 - \epsilon) \sum_{i=1}^k \ww_{H_i} (\partial_{H_i} (U)) \leq  \sum_{i=1}^k \ww_{G_i} (\partial_{G_i} (U)) = \ww_G (\partial_G (U)) \\ = \dots \leq (1 + \epsilon) \ww_H (\partial_H (U)) \, .
\end{multline*}
\end{proof}

\begin{lemma}
Assume there is a fully dynamic algorithm for maintaining a $ (1 \pm \epsilon) $-cut (spectral) sparsifier of size at most $ S (m, n, W) $ with worst-case update time $ T (m, n, W) $ for up to $ 4 n^2 $ updates in $ G $.
Then there also is a fully dynamic algorithm for maintaining a $ (1 \pm \epsilon) $-cut (spectral) sparsifier of size at most $ O (S (m, n, W)) $ with worst-case update time $ O (T (m, n, W)) $ for an arbitrary number of updates.
\end{lemma}

\begin{proof}
We exploit the decomposability of cut sparsifiers.
We maintain a partition of $ G $ into two disjoint subgraphs $ G_1 $ and $ G_2 $ and run two instances $ A_1 $ and $ A_2 $ of the dynamic algorithm on $ G_1 $ and $ G_2 $, respectively.
These two algorithms maintain a $ (1 \pm \epsilon) $-sparsifier of $ H_1 $ of $ G_1 $ and a $ (1 \pm \epsilon) $-sparsifier $ H_2 $ of $ G_2 $.
By the decomposability stated in \Cref{lem:decomposability cut sparsifier,lem:decomposability spectral sparsifier}, the union $ H \defeq H_1 \cup H_2 $ is a $ (1 \pm \epsilon) $-sparsifier of $ G = G_1 \cup G_2 $.

We divide the sequence of updates into phases of length $ n^2 $ each.
In each phase of updates one of the two instances $ A_1 $, $ A_2 $ is in the state \emph{growing} and the other one is in the state \emph{shrinking}.
$ A_1 $ and $ A_2 $ switch their states at the end of each phase.
In the following we describe the algorithm's actions in one phase.
Assume without loss of generality that in the phase are fixing $ A_1 $ is growing and $ A_2 $ is shrinking.

At the beginning of the phase we restart the growing instance $ A_1 $.
We will orchestrate the algorithm in such a way that at the beginning of the phase $ G_1 $ is the empty graph and $ G_2 = G $.
After every update in $ G $ we execute the following steps:
\begin{enumerate}
	\item If the update was the insertion of some edge $ e $, then $ e $ is added to the graph $ G_1 $ and this insertion is propagated to the \emph{growing} instance $ A_1 $.
	\item If the update was the deletion of some edge $ e $, then $ e $ is removed from to the graph $ G_i $ it is contained in and this deletion is propagated to the corresponding instance $ A_i $.
	\item In addition to processing the update in $ G $, if $ G_2 $ is non-empty, then one arbitrary edge~$ e $ is first removed from $ G_2 $ and deleted from instance $ A_2 $ and then added to $ G_1 $ and inserted into instance $ A_1 $.
\end{enumerate}
Observe that these rules indeed guarentee that $ G_1 $ and $ G_2 $ are disjoint and together contain all edges of $ G $.
Futhermore, since the graph $ G_2 $ of the shrinking instance has at most $ n^2 $ edges at the beginning of the phase, the length of $ n^2 $ updates per phase guarantees that $ G_2 $ is empty at the end of the phase.
Thus, the growing instance always starts with an empty graph $ G_1 $.

As both $ H_1 $ and $ H_2 $ have size at most $ S (n, m, W) $, the size of $ H = H_1 \cup H_2 $ is $ O (S (n, m, W)) $.
With every update in $ G $ we perform at most $ 2 $ updates in each of $ A_1 $ and $ A_2 $.
It follows that the worst-case update time of our overall algorithm is $ O (T (m, n, W)) $.
Furthermore since each of the instances $ A_1 $ and $ A_2 $ is restarted every other phase, each instance of the dynamic algorithm sees at most $ 4 n^2 $ updates before it is restarted.
\end{proof}


==> introduction-2.tex <==
\section{Introduction}

Dynamic algorithms provide a framework for the design of algorithms
that address situations in which the input is dynamically evolving. The goal is to maintain
 solutions that adapt to input updates but with a small amount of computational
 effort per update. Besides the theoretical questions underlying their design,
 dynamic algorithms are also well motivated by practice, as problems
 on very large dynamically evolving graphs (e.g. social networks,
road networks) become increasingly important.

It is then no surprise that recent years have seen a surge of interest in dynamic graph
algorithms. A number of key graph problems are now known to have efficient algorithms,
with polylogarithmic running time per update in the
graph (e.g.~\cite{HenzingerK99,HolmLT01,KapronKM13,OnakR10,NeimanS13,BaswanaGS15,BhattacharyaHI15,BaswanaKS12,AbrahamCDGW16}).
On the opposite end, recent work has also shown
strong conditional lower bounds for many basic problems~\cite{AbboudW14,HenzingerKNS15}.
In the face of such stubborn lower bounds, discovering new efficient dynamic
algorithms for natural graph problems is a major goal.

One can largely divide known efficient algorithms to
two classes: algorithms for problems with a distance or cut `flavor'.
In the distance case there are efficient
algorithms for fairly strong notions, such as approximate
planar shortest paths and
spanners. On the other hand,
in the cut case, known techniques seem to extend
only to more rudimentary (yet fundamental) problems,
such as connectivity, maximal matchings and MSTs.

In this paper we present the first efficient dynamic algorithm
for a very strong cut-based notion: \textbf{cut sparsifiers}~\cite{BenczurK15}.
These are sparse graphs that approximately preserve {\em all} cuts
of the input graph. We actually devise an efficient dynamic
algorithm for the even stronger notion of a \textbf{spectral sparsifier}~\cite{BatsonSST13}.
This is the first dynamic algorithm for a fundamental algebraic
problem.

Our spectral sparsification algorithm is inspired by the
spanner-based approach of Koutis~\cite{Koutis14}, and
naturally builds upon appropriately modified
dynamic spanner primitives that
provide an amortized update time upper bound~\cite{BaswanaKS12}.
Spectral sparsifiers are also cut sparsifiers.
Interestingly though, we are able to leverage
cut-based primitives, in particular the
recent breakthrough of Kapron et al.~\cite{KapronKM13},
to provide a different cut sparsification algorithm
with a \emph{worst case} upper bound on the update time.
This highlights a gap between the two notions
of sparsification,  which poses
an interesting problem. A similar gap in the streaming
model of computation has motivated significant recent research~\cite{KapralovLMMS14}.

Our main result for spectral sparsifiers is:
\begin{restatable}[]{theorem}{mainSpectral}
\label{thm:mainSpectral}
Given a graph with polynomially bounded edge weights,
we can dynamically maintain a $(1 \pm \epsilon)$-spectral sparsifier in
$poly(\log{n}, \epsilon^{-1})$ amortized time per edge insertion / deletion.
\end{restatable}
When used as a black box, this routine allows us to run cut
algorithms on sparse graphs instead of the original,
denser network.
Its guarantees interact well with most routines that compute
minimum cuts or solve linear systems in the graph Laplacian.
Some of them include:
\begin{enumerate}
\item mincuts, sparsest cuts, and separators~\cite{Sherman09},
\item eigenvector and heat kernel computations~\cite{OrecchiaSV12},
\item approximate Lipschitz learning on graphs~\cite{KyngRSS15} and a variety of matrix polynomials in the graph Laplacian~\cite{ChengCLPT15}.
\end{enumerate}

These routines and their extensions to the spectral setting~\cite{SpielmanT11,BatsonSST13}
play central roles in a number of recent algorithmic advances~\cite{Madry10,Sherman13,KelnerLOS14,PengS14,SpielmanTengSolver:journal,KyngLPSS15:arxiv,Peng16},
often leading to graph algorithms that run in almost-linear time.


In many applications the full power of spectral sparsifiers is not needed, and it suffices to work with a cut sparsifier. Our main result for cut sparsifier is:
\begin{restatable}[]{theorem}{mainCut}
\label{thm:mainCut}
Given a graph with polynomially bounded edge weights,
we can dynamically maintain a $(1 \pm \epsilon)$-cut sparsifier in
$poly(\log{n}, \epsilon^{-1})$ time per edge insertion / deletion in the worst case.
\end{restatable}



%As spectral approximations imply cut approximations,
%research in recent years has focused spectral sparsification
%algorithms~\cite{KelnerL13,KoutisLP12,KapralovLMMS14,ZhuLO15,LeeS15,JindalK15}.
%In the dynamic setting however we get a strictly stronger result for cut sparsifiers than for spectral sparsifiers: we can dynamically maintain cut sparsifiers with polylogarithmic \emph{worst-case} update time after each insertion / deletion.
%We achieve this by generalizing Koutis' sparsification paradigm~\cite{Koutis14} and replacing spanners with approximate maximum spanning trees in the construction.
%While there are no non-trivial results for maintaining spanners with worst-case update time, spanning trees can be maintained with polylogarithmic worst-case update time by a recent breakthrough result~\cite{KapronKM13}.
%This allows us to obtain the following result for cut sparsifiers:
% Previous text
%This routine goes through dynamic spanners, which have proven to be
%difficult to maintain in good worst case update time.\sebastian{We made this sentence a bit weaker because spanners with worst-case update time is not one of the big known open problems.}
%On the other hand, for cut sparsifiers, we can obtain worst case
%cut sparsifiers since all we need are spanning trees.


%motivated by graph cuts are well studied
%in theory and practice.
%The prevalence of large graphs motivated sublinear time
%algorithms for cut based problems such as
%clustering~\cite{SpielmanT13,BorgsBCT12,AndersenCL06,
%AndersenP09,OrecchiaV11,GharanT12}.
%In many cases such as social networks or road networks, these
%algorithms need to run on dynamically evolving graphs.

%As spectral approximations imply cut approximations,
%research in recent years has focused spectral sparsification
%algorithms~\cite{KelnerL13,KoutisLP12,KapralovLMMS14,ZhuLO15,LeeS15,JindalK15}.
%In the dynamic setting however we get a strictly stronger result for cut sparsifiers than for spectral sparsifiers: we can dynamically maintain cut sparsifiers with polylogarithmic \emph{worst-case} update time after each insertion / deletion.
%We achieve this by generalizing Koutis' sparsification paradigm~\cite{Koutis14} and replacing spanners with approximate maximum spanning trees in the construction.
%While there are no non-trivial results for maintaining spanners with worst-case update time, spanning trees can be maintained with polylogarithmic worst-case update time by a recent breakthrough result~\cite{KapronKM13}.
%This allows us to obtain the following result for cut sparsifiers:
% Previous text
%This routine goes through dynamic spanners, which have proven to be
%difficult to maintain in good worst case update time.\sebastian{We made this sentence a bit weaker because spanners with worst-case update time is not one of the big known open problems.}
%On the other hand, for cut sparsifiers, we can obtain worst case
%cut sparsifiers since all we need are spanning trees.


%motivated by graph cuts are well studied
%in theory and practice.
%The prevalence of large graphs motivated sublinear time
%algorithms for cut based problems such as
%clustering~\cite{SpielmanT13,BorgsBCT12,AndersenCL06,
%AndersenP09,OrecchiaV11,GharanT12}.
%In many cases such as social networks or road networks, these
%algorithms need to run on dynamically evolving graphs.

Dynamic cut sparsifiers turn out to be a crucial component
in more sophisticated applications, that we also discuss in  this paper.
A key property of these sparsifiers is that they have
arboricity $polylog(n)$.
This means the sparsifier is locally sparse, and
can be represented as a union of spanning trees.
This property is becoming increasingly important in recent
works~\cite{NeimanS13,PelegS16}:
Peleg and Solomon~\cite{PelegS16} gave data structures
for maintaining approximate maximum matchings on fully dynamic
graphs with amortized cost parameterized by the arboricity of the graphs.
We demonstrate the applicability of our data structures
for designing better data structures on the undirected
variant of the problem.
Through a two-stage application of graph sparsifiers,
we obtain the first non-separator based approach for
dynamically maintaining $(1 + \epsilon)$-approximate minimum
cuts on fully dynamic graphs:
\begin{restatable}[]{theorem}{mainBipartite}
\label{thm:mainBipartite}
We can maintain an $(1 - \epsilon)$ to the value of the maximum flow
on a dynamically changing unweighted, undirected,
bipartite graph, as well as query access to the associated minimum cut
in $poly(\log{n}, \epsilon^{-1})$ time per update.
\end{restatable}
To obtain this result we give stronger guarantees for vertex sparsification in bipartite graphs, identical to the terminal cut sparsifier question addressed by Andoni et al.~\cite{AndoniGK14}.
\richard{Changed these 2 sentences again}
Our new analysis profits from the ideas we develop by going back and forth
between combinatorial reductions and spectral sparsification.
This allows us to analyze a vertex sampling process via a mirror edge sampling
process, which is in turn much better understood.

Overall, our algorithms bring together a wide range of tools from
data structures,  spanners, and randomized algorithms.
We will provide more details on our routines, as well as how
they relate to existing combinatorial and probabilistic tools
in Section~\ref{sec:overview}.


==> introduction_r199.tex <==
\section{Introduction}

Dynamic algorithms provide a framework for the design of algorithms that address
situations in which the input is dynamically evolving. The goal is to maintain
solutions that adapt to input updates but with a small amount of computational
effort per update. Besides the theoretical questions underlying their design,
dynamic algorithms are also well motivated by practice, where problems
on very large dynamically evolving graphs (e.g. social networks,
road networks) become increasingly important. 

%\sebastian{Please check: added motivation for dynamic graph algorithms.}

It is then no surprise that recent years have seen a surge of interest in dynamic graph 
algorithms. A number of key graph problems are now known to have efficient algorithms,
with polylogarithmic running time per update in the 
graph 
(e.g. ~\cite{HenzingerK99,HolmLT01,KapronKM13,OnakR10,NeimanS13,BaswanaGS15,BhattacharyaHI15,BaswanaKS12,AbrahamCDGW16}).
On the opposite end, recent work has also shown
strong conditional lower bounds for many basic problems~\cite{AbboudW14,HenzingerKNS15}. 
In the face of such stubborn lower bounds, discovering new efficient dynamic
algorithms for natural graph problems is a major goal.

One can largely divide known efficient algorithms to
two classes: algorithms for problems with a distance or cut `flavor'. 
In the distance world there are efficient 
algorithms for fairly strong notions, such as approximate
planar shortest paths and
spanners. On the other hand, 
in the cut world, known techniques seem to extend
only to more rudimentary (yet fundamental) problems,
such as connectivity, maximal matchings and MSTs.

In this paper we present the first efficient dynamic algorithm
for a very strong cut-based notion: \textbf{cut sparsifiers}~\cite{BenczurK15}. 
These are sparse graphs that approximately preserve {\em all} cuts
of the input graph. We actually devise an efficient dynamic
algorithm for the even stronger notion of a \textbf{spectral sparsifier}~\cite{BatsonSST13}.
This is the first dynamic algorithm for a fundamental algebraic
problem. 

Our spectral sparsification algorithm is inspired by the
spanner-based approach of Koutis~\cite{Koutis14}, and 
naturally builds upon appropriately modified 
dynamic spanner primitives that
provide an amortized update time upper bound~\cite{BaswanaKS12}. 
Spectral sparsifiers are also cut sparsifiers. 
Interestingly though, we are able to leverage
cut-based primitives, in particular the
recent breakthrough of Kapron et al.~\cite{KapronKM13},
to provide a different cut sparsification algorithm
with a \emph{worst case} upper bound on the update time. 
This highlights an interesting gap between the two notions
of sparsification. 

\subsection{Main Results and Implications}

Our main result for spectral sparsifiers is:
\begin{restatable}[]{theorem}{mainSpectral}
\label{thm:mainSpectral}
Given a graph with polynomially bounded edge weights,
we can dynamically maintain a $(1 \pm \epsilon)$-spectral sparsifier in
$poly(\log{n}, \epsilon^{-1})$ amortized time per edge insertion / deletion.
\end{restatable}

When used as a black box, this routine allows us to run cut
algorithms on sparse graphs instead of the original,
denser network. Its guarantees interact well with most routines that compute
minimum cuts or solve linear systems in the graph Laplacian.
Some of them include:
\begin{enumerate}
\item min cuts, sparsest cuts, and separators~\cite{Sherman09},
\item eigenvector and heat kernel computations~\cite{OrecchiaSV12},
\item approximate Lipschitz learning on graphs~\cite{KyngRSS15} and a variety of matrix polynomials in the graph Laplacian~\cite{ChengCLPT15}.
\end{enumerate}

These routines and their extensions to the spectral setting~\cite{SpielmanT11,BatsonSST13}
play central roles in a number of recent algorithmic
advances~\cite{Madry10,Sherman13,KelnerLOS14,PengS14,SpielmanTengSolver:journal,KyngLPSS15:arxiv,Peng16},
often leading to graph algorithms that run in almost-linear time.

In many applications the full power of spectral sparsification is not needed, and it suffices to work with a cut sparsifier. %\sebastian{Please check: These sentences before the next theorem are new.}
We obtain the following result for cut sparsifiers.
\begin{restatable}[]{theorem}{mainCut}
\label{thm:mainCut}
Given a graph with polynomially bounded edge weights,
we can dynamically maintain a $(1 \pm \epsilon)$-cut sparsifier in
$poly(\log{n}, \epsilon^{-1})$ time per edge insertion / deletion in the worst case.
\end{restatable}

The gap between spectral and cut sparsification poses
an interesting problem. A similar gap in the streaming
model of computation has motivated significant recent research~\cite{KapralovLMMS14}. 

%As spectral approximations imply cut approximations,
%research in recent years has focused spectral sparsification
%algorithms~\cite{KelnerL13,KoutisLP12,KapralovLMMS14,ZhuLO15,LeeS15,JindalK15}.
%In the dynamic setting however we get a strictly stronger result for cut sparsifiers than for spectral sparsifiers: we can dynamically maintain cut sparsifiers with polylogarithmic \emph{worst-case} update time after each insertion / deletion.
%We achieve this by generalizing Koutis' sparsification paradigm~\cite{Koutis14} and replacing spanners with approximate maximum spanning trees in the construction.
%While there are no non-trivial results for maintaining spanners with worst-case update time, spanning trees can be maintained with polylogarithmic worst-case update time by a recent breakthrough result~\cite{KapronKM13}.
%This allows us to obtain the following result for cut sparsifiers:
% Previous text
%This routine goes through dynamic spanners, which have proven to be
%difficult to maintain in good worst case update time.\sebastian{We made this sentence a bit weaker because spanners with worst-case update time is not one of the big known open problems.}
%On the other hand, for cut sparsifiers, we can obtain worst case
%cut sparsifiers since all we need are spanning trees.


%motivated by graph cuts are well studied
%in theory and practice.
%The prevalence of large graphs motivated sublinear time
%algorithms for cut based problems such as
%clustering~\cite{SpielmanT13,BorgsBCT12,AndersenCL06,
%AndersenP09,OrecchiaV11,GharanT12}.
%In many cases such as social networks or road networks, these
%algorithms need to run on dynamically evolving graphs.

Dynamic cut sparsifiers turn out to be a crucial component
in more sophisticated applications, that we also discuss in  this paper.
A key property of these sparsifiers is that they have
arboricity $polylog(n)$.
This means the sparsifier is locally sparse, and
can be represented as a union of spanning trees.
This property is becoming increasingly important in recent
works~\cite{NeimanS13,PelegS16}:
Peleg and Solomon~\cite{PelegS16} gave data structures
for maintaining approximate maximum matchings on fully dynamic
graphs with amortized cost parameterized by the arboricity of the graphs.
We demonstrate the applicability of our dynamic sparsifiers
for designing better data structures on the undirected
variant of the problem.
Through a two-stage application of graph sparsifiers,
we obtain the first non-separator based approach for
dynamically maintaining $(1 + \epsilon)$-approximate minimum
cuts on fully dynamic graphs:
\begin{restatable}[]{theorem}{mainBipartite}
\label{thm:mainBipartite}
We can maintain a $(1 - \epsilon)$-approximation to the value of the maximum flow
on a dynamically changing unweighted, undirected,
bipartite graph, as well as query access to the associated minimum cut
in $poly(\log{n}, \epsilon^{-1})$ time per update.
\end{restatable}
To obtain this result we give stronger guarantees for vertex sparsification in bipartite graphs, identical to the terminal cut sparsifier question addressed by Andoni et al.~\cite{AndoniGK14}.
\richard{Changed these 2 sentences again}
Our new analysis profits from the ideas we develop by going back and forth
between combinatorial reductions and spectral sparsification.
This allows us to analyze a vertex sampling process via a mirror edge sampling
process, which is in turn much better understood.

Overall, our algorithms bring together a wide range of tools from
data structures,  spanners, and randomized algorithms.
We provide more details on our algorithms, as well as how
they relate to existing combinatorial and probabilistic tools
in Section~\ref{sec:overview}.

